Improving Schroeppel and Shamir's Algorithm for Subset Sum via Orthogonal Vectors

We present an $\mathcal{O}^\star(2^{0.5n})$ time and $\mathcal{O}^\star(2^{0.249999n})$ space randomized algorithm for solving worst-case Subset Sum instances with $n$ integers. This is the first improvement over the long-standing $\mathcal{O}^\star(2^{n/2})$ time and $\mathcal{O}^\star(2^{n/4})$ space algorithm due to Schroeppel and Shamir (FOCS 1979). We breach this gap in two steps: (1) We present a space efficient reduction to the Orthogonal Vectors Problem (OV), one of the most central problem in Fine-Grained Complexity. The reduction is established via an intricate combination of the method of Schroeppel and Shamir, and the representation technique introduced by Howgrave-Graham and Joux (EUROCRYPT 2010) for designing Subset Sum algorithms for the average case regime. (2) We provide an algorithm for OV that detects an orthogonal pair among $N$ given vectors in $\{0,1\}^d$ with support size $d/4$ in time $\tilde{O}(N\cdot2^d/\binom{d}{d/4})$. Our algorithm for OV is based on and refines the representative families framework developed by Fomin, Lokshtanov, Panolan and Saurabh (J. ACM 2016). Our reduction uncovers a curious tight relation between Subset Sum and OV, because any improvement of our algorithm for OV would imply an improvement over the runtime of Schroeppel and Shamir, which is also a long standing open problem.

==> Makefile <==
SOURCES := $(shell find $(SOURCEDIR) -name '*.tex')

all: main.pdf

main.pdf: $(SOURCES) main.bbl 
	pdflatex main.tex
	pdflatex main.tex

main.aux: $(SOURCES)
	pdflatex main.tex

main.bbl: bib.bib main.aux
	bibtex main

clean:
	rm -f img/*.log img/*.aux 
	rm -f *~ *.log *.out *.aux *.blg *.bbl *.gz

distclean: clean
	rm -f main.pdf

tar: clean
	bash -c "cd ..; tar -czf ${BASE}.tar.gz ${BASE}/*; mv ${BASE}.tar.gz ${BASE}"

spell:
	@for i in `find . -name "*.tex"` ; do \
		echo "------------ $$i --------------" ; \
		aspell list --lang=en --mode=tex --dont-tex-check-comments --personal=./blue-slownik.txt < $$i | sort | uniq ; \
done

diff:
	mkdir /tmp/equal-sums-diff/
	python2 ~/latex-flatten.py main.tex /tmp/equal-sums-diff/test.tex
	python2 ~/latex-flatten.py /tmp/equal-sums-diff/test.tex /tmp/equal-sums-diff/test2.tex
	python2 ~/latex-flatten.py /tmp/equal-sums-diff/test2.tex /tmp/equal-sums-diff/d2.tex
	git checkout $(branch-id)
	python2 ~/latex-flatten.py main.tex /tmp/equal-sums-diff/test.tex
	python2 ~/latex-flatten.py /tmp/equal-sums-diff/test.tex /tmp/equal-sums-diff/test2.tex
	python2 ~/latex-flatten.py /tmp/equal-sums-diff/test2.tex /tmp/equal-sums-diff/d1.tex
	latexdiff /tmp/equal-sums-diff/d1.tex /tmp/equal-sums-diff/d2.tex > /tmp/equal-sums-diff/diff.tex
	pdflatex /tmp/equal-sums-diff/diff.tex
	git checkout master

